Extreme Beam-forming with Impedance Metasurfaces Featuring Embedded Sources and Auxiliary Surface Wave Optimization

We present the end-to-end design of compact passive and lossless metasurface (MTS) antennas with integrated feeds. The complete low-profile system consists of a single-layered reactive impedance MTS printed on top of a grounded dielectric substrate, and is fed by sources which are embedded inside the substrate. An accurate and efficient volume-surface integral equation-based model of the device is developed, and used as the basis for the rapid optimization of its performance. The optimized designs leverage tailored auxiliary surface waves supported by the impedance MTS to distribute the localized source power across their apertures. This facilitates the realization of extreme field transformations such as wide-angle beam-forming or shared-aperture beam-forming, with nearly 100% aperture efficiencies. The procedure also allows for arbitrary beam-shaping with complete main beam and side lobe control. We also derive several feasibility-related constraints, which can significantly enhance the power efficiency as well as the bandwidth of the MTS antennas when they are implemented in practice. Full-wave numerical simulations confirm the effectiveness of the presented approach, as well as the extreme field transformation capabilities of the synthesized designs.

==> Scratch.tex <==
\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By varying the abstract surface impedance $Z_w$ of this wire and leveraging the method of moments formulation developed in Sec.~\ref{sec:model}, the predicted total electric field at a near-field observation segment close to this single-wire device can be recorded and stored. Then, a simulation is conducted in HFSS with realistic printed wires, and the obtained actual total field along this observation segment is compared against the predicted electric field for different values of $Z_w$. We pick the value of $Z_w$ corresponding to the best overall matching is the one picked as the extracted impedance value. This method characterizes the capacitive loadings taking into account the dielectric and the ground plane that will be present in the final metasurface antenna. 

{\color{red} Perhaps we should remove this paragraph. It could create some confusion, and I'm not sure if Popov's method is really necessary. Also we don't really need this I think.}
\hl{Alternatively, simulations with the local periodic assumption could have been performed. With this method, the wire is placed inside an infinitely periodic surrogate model, which is then illuminated by a plane wave. The value of the reflection coefficient is utilized to infer the wire loading. However, one needs to manually remove the effect of the other wires in the infinite array}~\cite{Popov:PRA2019} \hl{as well as that of the grounded dielectric, in order to be in alignment with the framework presented in Sec.~{\ref{sec:model}}.}
\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To determine the desired far-field radiation, we assume a number of virtual sources along the ground plane. The current of these sources is calculated as the superposition of two uniform-amplitude distributions as follows:
\begin{align}
J_n= A_1 e^{-j k_0 \mathrm{sin} (\theta_1) n \Delta y}+A_2 e^{-j k_0 \mathrm{sin} (\theta_2) n \Delta y} e^{j \xi},
\end{align}
\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
